Benchmarking Machine Translation with Cultural Awareness

Translating culture-related content is vital for effective cross-cultural communication. However, many culture-specific items (CSIs) often lack viable translations across languages, making it challenging to collect high-quality, diverse parallel corpora with CSI annotations. This difficulty hinders the analysis of cultural awareness of machine translation (MT) systems, including traditional neural MT and the emerging MT paradigm using large language models (LLM). To address this gap, we introduce a novel parallel corpus, enriched with CSI annotations in 6 language pairs for investigating Culturally-Aware Machine Translation--CAMT. Furthermore, we design two evaluation metrics to assess CSI translations, focusing on their pragmatic translation quality. Our findings show the superior ability of LLMs over neural MTs in leveraging external cultural knowledge for translating CSIs, especially those lacking translations in the target culture.

==> sections/01_introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}
% \junjie{Potential outline: (1) Recent years have witnessed the success of multilingual MT systems over diverse language pairs, especially with the advent of multilingual pre-trained language models. We have observed encouraging cross-lingual transfer results that improve the translation of low-resourced languages. (2) However, the cross-lingual transfer a\input{sections/01_introduction}bility of MT systems does not necessarily imply the cross-cultural understanding ability. As most MT systems are built to still optimize performance on certain coarse automatic metrics such as BLEU, and BERTScore, there is a lack of methods for optimizing the cross-cultural awareness of MT systems. Moreover, there is no systematic study to evaluate the cultural awareness of MT systems across languages. (3) Point out the limitation of current methods in terms of datasets, modeling, and evaluation perspectives. 3.1 Most MT datasets consist of parallel texts and do not contain culture-specific annotations. 3.2 (TBD) Existing data-driven MT models still heavily rely on massive training data, while cultural mentions are often low-frequency entities. As a result, even commercial MT systems still make errors across cultures. \binwei{The same problem also arises when using GPT models such as ChatGPT for translation tasks.} 3.3 As culture differences are usually very subtle, misinterpreting culture-specific entities is the most common error that existing evaluation metrics cannot easily capture. As shown in Figure 1 \binwei{TBD: A figure showing errors of google and ChatGPT} (4) (new paragraph) To address these challenges, we conduct a comprehensive study to understand the cultural awareness of MT systems. Describe our dataset construction pipeline. Introduce a few baselines and our methods to mitigate this issue. Showcase our performance using our fine-grained evaluation methods. (5) Highlight several potential research questions moving forward and shed new insights on potential solutions to improve cultural awareness. }



% \junjie{Outline: 1. NMT models have achieved good results in many language pairs. However, their translation performance on culturally sensitive data is still poor, due to the gap between the cultural backgrounds of the language users. As languages and culture are highly-intertwined, it is essential that MT systems should bridge the cross-cultural gab between a source-target language pair and produce understandable translations to the target audience.  }
% Translating cultural-specific terms is essential for cross-culture communication~\cite{fernandez2012translating}.
%\junjie{Let me write the outline here: 1. First paragraph: CSI translation is difficult, because of a) lack of data resources; and b) lack of evaluation methods. 2. most existing terminology data resources focus on popular domains such as medicine or finance, yet not much on CSI. 3. evaluating CSIs is different. CSIs may not have translations, therefore this requires us to generate explanation-based translations that are more understandable to target-language speakers. 4. (New paragraph) LLM-MT opens up such an opportunity to generate explanation-based MT and allows us to easily integrate external knowledge. Compared to traditional terminology methods, it's less prone to overfitting, and doesn't require further training. 5. However, its performance comparisons to traditional NMTs is still unknown. 6. (New paragraph) To tackle these issues, we propose this data curation method, the resources, and the evaluation methods -- summarizing the three contributions and key findings. }


\begin{figure}[t]
    \centering   \noindent\includegraphics[width=\columnwidth]{figures/motivating_example_GPT4o.pdf}
    \caption{Cultural Translation Errors Made by GPT-4o}
    \label{fig:examples}
    % \vspace{-5mm}
\end{figure}

% Why translating CSIs is important for MT systems?
Machine translation (MT) systems, as important cross-culture communication tools \cite{liebling2020unmet}, have achieved remarkable success in recent years, thanks to multilingual pre-trained language models~\cite{aharoni-etal-2019-massively}. However, MT systems' semantic alignment objective is not sufficient for cross-culture translation~\cite{hershcovich2022challenges}, where further adaption to the target culture is necessary~\cite{vinay1995comparative}. Therefore, their translation performance on culturally specific data is still poor~\cite{akinade-etal-2023-varepsilon, liebling-etal-2022-opportunities}. The variation of cultural-specific-items has been a long-standing aspect of translation studies~\cite{newmark1988textbook, persson2015culture,fernandez2012translating}.
Many cultural-specific concepts in various categories (e.g., food, clothing, art, religions) are not frequently used by users across other cultures~\cite{woolford1983bilingual}, which can make their semantic equivalences in other languages confusing or even misleading. For example, in Figure~\ref{fig:examples}, GPT-4o translates ``En Vogue'' into its transliteration ``\begin{CJK}{UTF8}{gbsn}恩沃格\end{CJK}'' in Chinese, which resembles a personal name, whereas ``En Vogue'' actually refers to a vocal girl group.

% Relate work summary and challenges of use these methods in translating CSIs
Previously, there are lots of efforts in improving translation quality of terminology \cite{dinu2019training, ghazvininejad2023dictionary}. However, existing terminology translation datasets and methods mostly focus on popular domains (e.g., medicine, finance)~\cite{dinu2019training,ghazvininejad2023dictionary}, yet do not cover much on cultural-specific aspects. 

% The Challenges of research
To bridge the gap, our research aims to have a systematic study in MT systems ability in translating CSIs, which mainly has three challenges: 1) data scarcity; 2) evaluation method insufficiency; 3) cultural knowledge integration in translation.

% Distinguished from general terms, cultural-specific items are unique to particular cultural groups, making their transliterations and literal translations difficult for people from other cultures to understand. 
% Moreover, many CSIs have no translations into other languages, further increasing the difficulty of data collection and evaluation of the translation performance. For example, in Figure~\ref{fig:examples}, a Taiwanese dish called ``\begin{CJK}{UTF8}{gbsn}五更肠旺\end{CJK}'', which is chitterling in hot pot, has no well-known existing English translations. The translation of ChatGPT ``Five-spice intestines and blood curd'' is misleading and can not be easily understood by English native speakers. In contrast, a professional human translator would elicit an explanation to make the translation more understandable for readers.
% As a result, the nuanced characteristics of CSIs and the limited availability of data sources pose challenges in building culture-aware MT systems that can translate these terms into accurate and understandable ones in target languages.

% Early work on terminology translation focuses on integrating external knowledge, like lexicon translation, into MT systems through probability interpolation~\cite{arthur-etal-2016-incorporating,khandelwal2021nearest}, data augmentation~\cite{hu-etal-2019-domain-adaptation}, and pre-training~\cite{hu-etal-2022-deep}. One major concern with these methods is that fine-tuning the pre-trained MT models with external knowledge may cause new issues like catastrophic forgetting~\cite{thompson-etal-2019-overcoming}. Moreover, the injected knowledge is static in model deployment, making it hard for the models to address cultural knowledge outside of the injected one. \junjie{I would suggest delete this paragraph.}

% What's opportunities and challenges of LLM-based MT for CSIs?
% Recently, a new translation paradigm has emerged, which employs prompts to guide large language models (LLMs) to perform machine translation~\cite{gpt3} in a zero-shot or few-shot fashion. With this flexible paradigm, cultural knowledge can be seamlessly incorporated into LLM translation prompts. \binwei{Challenges}

% However, LLM-based translation is sensitive to prompting strategies and prone to generating hallucinations~\cite{ji2023survey}. 
% % As shown in Figure~\ref{fig:examples}, the translation of ``A Few Good Men'' as ``\begin{CJK}{UTF8}{gbsn}壮志凌云\end{CJK}'' (i.e., Top Gun) wrongly refers to a completely different film. 
% Given that, the cultural sensitivity of LLM-based MT systems remains an open question, especially when dealing with culturally relevant content. Moreover, there is scant research comparing LLM-based translation versus NMT systems regarding their cultural awareness, partly due to the absence of a rich-annotated culturally sensitive parallel corpus and reliable automated metrics for evaluation. This scarcity further hinders the MT development in navigating cultural nuances, limiting the MT systems' efficacy in promoting cross-cultural communication.
%Languages and culture are highly intertwined~\cite {gee2014introduction,kramsch2014language}, thus many cultural-specific concepts in various categories (e.g., food, clothing, art, religions) are not frequently used by users across other cultures~\cite{woolford1983bilingual}. 



%One solution to address the aforementioned issue is integrating external cultural knowledge, such as lexicon translation, into MT systems through probability interpolation~\cite{arthur-etal-2016-incorporating,khandelwal2021nearest}, data augmentation~\cite{hu-etal-2019-domain-adaptation}, and pre-training~\cite{hu-etal-2022-deep}. \binwei{However, these methods require additional fine-tuning on the original Neural MT (NMT) models, potentially resulting in new issues such as catastrophic forgetting~\cite{thompson-etal-2019-overcoming}, and can not easily inject external knowledge except dictionaries during test time.} 




%These mistranslations can be challenging to comprehend, as they may involve incorrect word order or misleading references. For example, the translation of ``egg foo young'' as ``\begin{CJK}{UTF8}{gbsn}炒蛋芙蓉\end{CJK}'' misplaces the translations of ``egg'' and ``foo young'', and the translation of ``A Few Good Men'' as ``\begin{CJK}{UTF8}{gbsn}壮志凌云\end{CJK}'' refers to a completely different film.
% like ``egg foo young'''s translation `` \begin{CJK}{UTF8}{gbsn}炒蛋芙蓉\end{CJK}'', which misplaces translations of ``egg'' and  ``foo young'', or generate misleading references, such as ``A few Good Men'''s translation ``\begin{CJK}{UTF8}{gbsn}壮志凌云\end{CJK}'', which refers to another different film.

% In this work, we examine the cultural awareness of a series of MT systems, including LLM-based MT systems, traditional NMT systems, and commercial MT systems on 6 language pairs, including English-Chinese, English-French, English-Spanish, English-Hindi, English-Tamil, and English-Telugu. 

% In this study, we focus on addressing two research questions: (1) NMT vs. LLM-based MT, which group of MT systems embed more cultural awareness? (2) Diving into LLM-based MT, what prompting strategy benefits the most for guiding LLMs in cultural-specific translation?
To tackle these challenges, we propose a novel data curation pipeline to build a culture-centered parallel corpus with limited human annotation efforts. To capture challenging examples with geo-metadata, we further conduct cultural knowledge augmentation for CSIs. Our parallel corpora include \textbf{6 language pairs} (i.e., English-Chinese, English-French, English-Spanish, English-Hindi, English-Tamil, and English-Telugu), covering \textbf{7,253 CSIs in 18 concept categories from over 140 countries and regions.}

%Specifically, referring to a well-established classification framework on cultural-specific items (CSIs i.e., entities that are unique to a specific culture) ~\cite{newmark1988textbook}, we build a cultural taxonomy to identify culturally relevant texts from parallel corpora. 

% Overall, we collect \textbf{1,140 English-Chinese sentence pairs} involving different \textbf{573 CSIs} across \textbf{18 concept categories} in \textbf{21 countries}. 
% Overall, we collect \textbf{1,140 English-Chinese sentence pairs} involving different \textbf{573 CSIs} across \textbf{18 concept categories} in \textbf{21 countries}. 


To assess the cultural nuance, we design new automatic metrics targeting the translation quality of cultural concepts, both on the translation accuracy and understandability. Different from existing evaluation metrics which mainly focus on semantic similarity with the reference~\cite{anastasopoulos2021evaluation}, we define a new metric called \textit{understandability} to evaluate the CSI translation in a reference-free manner. We use our metrics to compare a series of MT systems, including LLM-based MT, traditional NMTs, and commercial MT systems, on translating cultural content. Moreover, we examine a set of prompting strategies to endow cultural knowledge into LLM-based MT. The traditional terminology translation method enhances the accuracy of translating CSIs that have well-known references but falls short of translating no-translation CSIs. However, incorporating CSI explanations in the prompt significantly improves the translation quality, especially for no-translation CSIs. Our further investigation into different MT systems' translation strategies reveals that employing more sophisticated approaches, such as describing CSIs and substituting them with similar content in the target language, effectively improves the readability of CSI translations. %Lastly, we analyze the translation mechanisms employed by different MT systems when translating cultural content, which, coupled with human evaluations, seeks to facilitate future enhancement and evaluation of cultural awareness of MT systems. 
In summary, our contributions are:

%referring to a well-established classification schema on cultural-specific item (CSI) ~\cite{newmark2003textbook}, we constructed a cultural taxonomy to identify culturally relevant texts from Wikipedia. 
%, which serves as a valuable resource for evaluating the cultural awareness of MT systems. 
% We further augmented the data and capture challenging examples by adversarial mining. %The pipeline involves collecting parallel texts including entities from culture-related Wikipedia categories, augmenting the knowledge with Wikidata metadata, and using adversarial mining to identify challenging examples for translation engines.
% Our pipeline starts with constructing a cultural taxonomy that is used to identify culturally relevant texts from Wikipedia and then performs adversarial mining to further select culturally nuanced texts. 
%Our parallel corpus \textbf{has 1,140 English-Chinese sentence pairs} in total, which \textbf{contains 1,148  cultural-specific items}, \textbf{covering 18 Wikipedia categories across 21 countries}. 



\begin{itemize}[leftmargin=13pt]\itemsep-0.2em
    % \item We construct cultural-specific parallel corpora of 6 language pairs with rich cultural-related annotations, enabling a fine-grained evaluation of popular MT systems on their cultural awareness.
    % \item We conduct fine-grained automatic and human evaluations on the culture-awareness of a series of MT systems.
    % \item We introduce simple yet effective prompting strategies using \textit{external knowledge} and \textit{internal knowledge} for LLM-based machine translation and systematically benchmark their performances on our culturally specific corpus.
    % \item We offer new insights into enhancing the cultural awareness of LLM translation based on our automatic evaluation metric and fine-grained analysis.
    \item We introduce a novel data curation pipeline for constructing a culturally relevant parallel corpus, enriched with annotations of culturally specific items.
    \item We develop two metrics for translation quality: CSI-Match, which evaluates accuracy for well-known translations, and Understandability, which addresses cultural nuances beyond accuracy, especially for terms lacking established translations.
    \item We assess various NMT and LLM-based MT systems using our dataset and metrics. Results show that while traditional NMT models excel in semantic matching, they often struggle with comprehensibility of culturally specific items.
    \item We suggest cultural knowledge prompting strategies to improve understandability through external knowledge integration, demonstrating promising results.
\end{itemize}



==> sections/03_models.tex <==
\section{Cultural Knowledge Prompting}
\label{sec:culture_mt}

In this section, we explore various prompting strategies to introduce cultural knowledge for LLM MT. 
% A prompt for LLMs typically consists of a natural language task description accompanied by few-shot in-context examples. 
We elucidate our strategies for generating in-context examples from \textit{external knowledge}, which involve employing CSI translation pairs and CSI explanations. Additionally, we delve into several prompting strategies eliciting from LLMs' \textit{internal knowledge}. Table~\ref{tab: Prompting Strategy} shows examples of various prompting strategies.
%\junjie{This will be the main technical section to show the prompting methods that we've tried in this study. }
\input{tables/16_prompting_examples}
% \input{tables/01_examples}

% \subsection{Source v.s. Target Language Instructions}
% \label{sec:instruct_lang}
% % \junjie{Add the description of comparing the source and target languages used for task description}
% As LLMs have been pre-trained on massive texts in multiple languages, their capability of interpreting instructions in different languages has not been comprehensively studied for machine translation. We hypothesize that the language used in the prompt has an impact on the language model's understanding of the instructions and the demonstrations.
% % and the target language will bias the model to better leverage the information in the prompt for machine translation tasks. 
% Thus, we propose to construct prompts in the source and target languages and compare the LLMs' translation performance of CSIs.

\subsection{External CSI Translation (CT)}
\label{sec:ent_translate}
% \junjie{Add the description about constructing the entity translations as part of the prompt here.}
We examine an external CSI dictionary for improving LLM-based MT. 
In particular, bilingual translation dictionaries play a vital role in the workflow of human translators~\cite{ghazvininejad2023dictionary}. 
% Professional translators often compile domain-specific terminology dictionaries, enabling them to maintain consistency while translating the terminologies within a specific domain. 
% Historically, it is non-trivial to integrate the translation dictionary into neural machine translation models~\cite{arthur-etal-2016-incorporating,hu-etal-2019-domain-adaptation}, compared to phrase-based machine translation systems. However, with the advent of large language models (LLMs) for machine translation, incorporating entity information into prompts has become much more feasible. 
% Existing research also shows that word dictionaries would be helpful for low-resource or domain transfer machine translation~\cite{ghazvininejad2023dictionary}.
Here, we assess the impact of incorporating a CSI dictionary within the prompts. Specifically, we incorporate CSIs along with their corresponding translations prior to a basic translation instruction. 

% This methodology allows us to investigate the potential benefits of leveraging a CSI dictionary in LLM-based translation models.


\subsection{External CSI Explanation (CE)}
\label{sec:ent_explain}
% \junjie{Add the description about constructing the entity explanation from WikiData/Wikipedia}
CSIs may not have a direct equivalent in the target language's culture when the concepts are not commonly used by the target language speakers. Therefore, it becomes necessary to translate based on the explanation of the CSI to assist the target audience in better understanding the content. To assess the impact of explanations, we include the CSI description obtained from Wikipedia in the prompt before the basic translation instructions. This allows us to study whether additional explanations of CSIs can enhance the MT performance.



\subsection{Self-Explanation (SE)}
% \junjie{We may compare whether the LLM can automatically generate the entity translation by itself here. That is, similar to Zero-shot CoT (by adding ``let's think step by step'', we can add an extra instruction like ``Let's translate/explain the cultural entities in the text one by one'', and then collect the LLMs' response to prompt the LLM to do the translation.}
We also examine LLMs' \textit{internal knowledge} for explaining the meaning of CSIs. Notably, Chain-of-Thought (CoT) prompting has shown effective in eliciting LLMs' internal knowledge~\cite{wei2022chain,kojima2022large}. Inspired by this, we treat the explanation of CSIs in a source sentence as intermediate reasoning steps before translating the whole sentence. We then design the explanation prompting strategy in two steps for machine translation. In the first step, we prompt the LLM to explain the meaning of all CSIs in the source sentence.
% by using a prompt template, i.e., ``\textit{Please explain [CSI] in [Source Sentence]}.'' 
In the second step, we ask the LLM to translate the whole sentence by combining the LLM's explanation with another prompt instruction.
% i.e., ``\textit{According to your explanation to [CSI], only translate the following [Source Language] text to [Target Language]: [Source Sentence]}.'' 

% By comparing self-explanation with external CSI explanations (\Scref{sec:ent_explain}), we aim to examine how well LLMs can understand the cultural nuances of the CSIs in the sentence context.
%using CoT prompting, we aimed to provide the LLMs with a more structured and contextually rich input, which would help it reason more effectively about the cultural nuances of the CSIs.

% \subsection{Self-Correction (SC)}
% It has been shown that LLMs can correct their own mistakes if instructed to perform generations with specified constraints~\cite{ganguli2023capacity}.  Building upon this finding, we investigate the potential benefits of self-correction in the translating of CSIs within sentence content. Specifically, to encourage the LLM to identify the target-language culture for native speakers, we design the following instruction: \textit{``Please firstly think about how to ensure that the culturally relevant words in the sentence are translated into [Target Language] words that [Target Language] readers can understand.''}. In the first step, we prompt the LLM with the basic translation instruction plus the instruction to enable the LLM to generate analysis to achieve the goal. Next, we ask the LLM to translate the whole sentence according to its analysis.
% % i.e., ``\textit{According to your analysis, please translate the sentence.}'' This allows LLM to analyze the translation approach for culturally related content and adjust translation results based on its analysis.

% % conducted two experiments: one using the Instruction Following (IF) method and another using IF combined with the Chain-of-Thought (COT) method. For the translation task of CSI, we design the following instruction as "ensure that the culturally relevant words in the sentence are translated into Chinese words that can be understood by Chinese readers".

\subsection{Self-Ranking (SR)}
Finally, LLMs can be prompted to sample different translation outputs. Even for multiple semantically equivalent prompts, the word choice in the prompts can have a significant impact on the performance of LLM models in translation tasks. To achieve more consistent and reliable results, we examine a self-ranking method~\cite{wu2023improving} to instruct LLMs to rank their translation outputs. Specifically, we prompt the model to first generate a fixed number of potential translations. 
% % The Generated Number is a hyper-parameter for the number of translations to generate. 
% Subsequently, we ask the LLM select the most optimal one according to our predetermined optimization goal for cultural awareness, i.e, ``\textit{the meaning of the word is easy to be understood by [Target Language] readers''}. 

% The performance of LLM models in translation tasks can be significantly influenced by the choice of prompt. To ensure more consistent and reliable results, we employed the self-ranking method, which involves the model generating multiple potential translations and then selecting the most optimal one based on our predetermined optimization goals. This approach helped to improve the stability and accuracy of the model's translations.

==> sections/05_results_old.tex <==
\section{Results and Analysis}
\label{sec:results}
Our analysis includes three parts: 1) automatic evaluations between LLM-based translation and popular NMT systems (\Scref{sec:auto_eval}) on six language pair translations; 2) assessing LLM prompting strategies using ChatGPT and LLaMA for En-to-Zh translation (\Scref{sec:prompting_auto_eval}); and 3) fine-grained human evaluation on a subset of En-to-Zh pairs (\Scref{sec:human_evaluation}).
%Our study of culture-awareness in MT systems includes three parts. First, we apply automatic evaluations to compare the LLM translation with existing popularly-used MT systems (\Scref{sec:auto_eval}). Then, we evaluate different LLM prompting methods using ChatGPT and LLaMA for English-to-Chinese translation (\Scref{sec:prompting_auto_eval}). Lastly, we perform a fine-grained human evaluation on a subset of English-to-Chinese pairs to comprehensively compare the performances of various MT systems (\Scref{sec:human_evaluation}).

\subsection{Overall Automatic Evaluation}
\label{sec:auto_eval}
% \input{tables/02_chinese_auto_evaluation}
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
         % \centering
         \includegraphics[width=\textwidth]{figures/csi-match-1.pdf}
         % \includegraphics[width=0.42\textwidth]{figures/csi-match-2.pdf}
         \caption{Traditional MT Systems}
         \label{fig:nmt csi-match}
         % \vspace{-3mm}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/csi-match-2.pdf}
         \caption{LLM-based MT Systems}
         \label{fig:llm csi-match}
         % \vspace{-3mm}
     \end{subfigure}
    % \includegraphics[width=0.45\textwidth]{figures/csi-match-1.pdf}
    \caption{CSI-Match on Different Language Pair Translations: The coordinate scale range is from 40 to 100.
    % \junjie{is it visually better/compact to put the two figures and Table 4 in a single row over two text columns using latex's ``minipage'' package}
    }
    \label{fig:cs-match-languages}
    \vspace{-3mm}
\end{figure}
\input{tables/13_understandability}

\paragraph{Replacement and Append Work for NLLB and LLM-MT in CSI-Match.}
% \junjie{6.1 A figure to show the CSI-match on 8 methods. Findings: 1. simple strategies (like replacement, append) can work on metrics based on string match (CSI-match, and others in the appendix). 2. LLM-MT can leverage dictionary appending in the prompt. }
Figure \ref{fig:cs-match-languages} shows the CSI-Match scores (\Scref{sec:culture_mt_evaluation}) for eight methods across cultural-related parallel corpora in six language pairs, which are collected by our pipeline (\Scref{sec:dataset}). Figure~\ref{fig:nmt csi-match} shows the CSI-Match scores of traditional MT systems including vanilla NLLB, NLLB-A, NLLB-R, and Google Translate, whereas Figure~\ref{fig:llm csi-match} shows scores of LLM-based MT systems including LLaMA2, LLaMA2-A, LLaMA2-R and ChatGPT. We find that straightforward strategies using dictionaries of CSIs, such as Replace~(the \textcolor[HTML]{2ca02c}{green} solid line) and Append (the \textcolor[HTML]{ff7f0e}{orange} solid line), are effective on metrics that rely on string-matching, such as CSI-match, as well as other semantic matching metrics detailed in Appendix \Scref{sec:overall_auto_metric}. However, the appending strategy significantly benefits LLaMA more than NLLB. This suggests that LLaMA's capacity of in-context learning and instruction-following enables the flexible integration of cultural knowledge at test time, a capability not presented in traditional NMT systems like NLLB. %Achieving the same level of adaptability in the latter is considerably more challenging. 
Additionally, we measure the CSI-Match of ChatGPT using basic instructions (BI), and Google Translate (the \textcolor[HTML]{d62728}{red} solid line). We find that Google Translate's performance across different languages is generally more consistent compared to ChatGPT. Specifically, Google Translate performs better in non-Latin languages such as Chinese, Hindi, Tamil, and Telugu, when compared to ChatGPT.


 %For LLaMA2-R, we replace the CSIs in Source Sentences by their corresponding translation in target language.

\paragraph{Understandability Gap on Non-translation CSIs}
% \junjie{However, if we take a look at understandability, these methods still have a gab in translating CSIs, especially for those without the reference translation. }
Table \ref{tab: Understandability by GPT-4} presents the understandability win rates assessed by GPT-4 for various MT systems compared to the reference in English-Chinese translation. Appendix \Scref{sec:evaluation_prompts} has the detailed evaluation prompt. The evaluation metrics include both the overall win rates across the entire dataset (\textbf{Overall-U}) and the win rates of samples containing complex source items (CSIs) with no translations (\textbf{NT-U}). The results indicate that traditional terminology translation methods, such as Appending and Replacing, effectively improve the overall understandability across the entire dataset. However, they still encounter challenges in improving the comprehensibility of translations that contain CSIs without a well-established reference. Notably, ChatGPT performs better than any other MT systems, which potentially suggests that the instruction-tuning of LLMs beyond the translation task may be beneficial for the model to generate explanation-based translations for these non-translation CSIs.

\subsection{Prompting Strategy Evaluation}
\label{sec:prompting_auto_eval}
\input{tables/14_understandablity_prompting}
% \junjie{6.2 LLM-MT offers the option to generate free-form explanations, opening opportunities to improve understandability. So we investigate different prompting strategies to include additional culture information.}

As LLM-based MTs open up the opportunity to incorporate free-form external knowledge for improving the understandability of non-translation CSIs, we explore various prompting strategies by incorporating additional cultural information alongside dictionaries to improve translation. We compare different prompting strategies on ChatGPT, focusing on English-to-Chinese translation. We examine both zero-shot and 2-shot approaches to obtain results from ChatGPT. Especially for complex prompting strategies including CE, SE, and SR, we use 2-shot examples that are tailored for culturally-aware translation.
Table~\ref{tab:understandablity_prompting_methods} shows the results of different prompting methods. 

\paragraph{External Knowledge Prompting} Comparing the strategy of using external knowledge in prompts (i.e., CT and CE), we observe that LLMs can effectively leverage both direct translations and indirect descriptions. Specifically, CT greatly enhances the CSI-Match score for CSI translation. While 2-shot CE demonstrates limited improvements on CSI-Match, it improves the overall understandability of the entire dataset. More importantly, 2-shot CE significantly improves the non-translation CSIs' understandability to 73.0. This suggests that CSI explanations offer significant assistance in translating CSIs, especially for the ones without well-known translations. In Table \ref{tab: Prompting Strategy Examples}, we quantitatively show the output examples of ``Polenta,'' an Italian corn porridge. Interestingly, its Chinese translation on Wikidata is merely a transliteration. Under the CT strategy, ChatGPT directly copies this transliteration into the output, which may be considered correct yet not comprehensible for native speakers of the target language. In contrast, ChatGPT using CE integrates an explanation into the translation, describing the CSI as ``corn porridge'' in Chinese. This translation is much easier for readers to understand the nature of Polenta.

\paragraph{Internal Knowledge Prompting} Next, we compare prompting strategies to elicit LLMs’ internal knowledge (i.e., SE, SR). We find that 2-shot SE improves translation performance on CSI-Match and Overall-U but doesn't improve the NT-U, which suggests that ChatGPT itself still lacks sufficient knowledge of non-translation CSIs which are typically very unique to the target-language culture. On the other hand, SR proves beneficial on ChatGPT for CSI-Match but does not improve the understandability of CSI translations, indicating that LLMs inherently possess internal knowledge of low-frequency CSIs but still can not capture cultural nuances through the SR prompting strategy examined in this study. 
In Table~\ref{tab: Prompting Strategy Examples}, 2-shot SR translates ``Polenta'' as ``cornmeal,'' similar to the baseline (BI). However, SE successfully translates it into ``corn porridge.'' This suggests that ChatGPT possesses background knowledge of Polenta but struggles to spontaneously elicit it to generate and select the most understandable translations.
% \junjie{SE is 2-shot, but SR here is zero-shot? The last sentence is not fair.}
\input{tables/17_prompting_result_examples}


\subsection{Human Evaluation}
\label{sec:human_evaluation}

% To provide a fine-grained assessment regarding the understandability of the CSI translations (\Scref{sec:culture_mt_evaluation}), we conduct a human evaluation of our selected MT systems (LLaMA, NLLB, ChatGPT, and Google) on 200 English-to-Chinese translation examples. We ask a Chinese native speaker to rank the understandability of the 4 MT system's translations.
% Table \ref{tab: Undertandability Ranking Results} shows the ranking results. Google Translate still performs the best in understandability, followed by ChatGPT. NLLB performs slightly better or comparable to LLaMA.
\paragraph{GPT-4 and Human Evaluation Are Consistent.} 
Table \ref{tab:consistency} shows the Overall-U evaluated by both GPT-4 and human annotators. Specifically, we randomly select 200 samples from the English-to-Chinese translation dataset and have human annotators evaluate the understandability of output translations by the four different methods. The results indicate a high level of consistency between human annotations and GPT-4's evaluations
\input{tables/15_consistency}


To compare the consistency between automatic and human evaluation, we also calculate the correlation between automatic evaluation metrics and human evaluation, where we consider the translation correct in human evaluation if the translation is categorized into all the translation strategies except Copy and Wrong. The Pearson's correlation between the human evaluation and BLEU, BLEURT and COMET are 88.8, 90.5, and 89.5 respectively, whereas CSI-Match has the highest correlation score at 94.7 with human evaluation, suggesting that CSI-Match can be an efficient evaluation metric for CSIs with a reference translation. 

% \binwei{add consistency analysis of GPT4}
% % \input{tables/10_understandablity_stats}


% In addition, we also ask the native Chinese speaker to categorize the system outputs into 4 groups: 1) correct where the system outputs match one of the translation references; 2) copy where the system copies the source CSI as output; 3) understandable where the system generates an understandable CSI translation instead of the reference translation; 4) wrong where the system output is completely wrong. We show the distribution of categories from all baseline models and LLM-based MT with different prompting strategies in Figure \ref{fig:human_evaluation}.






% \input{tables/06_correlation}
% Old Version

%In this section, we first compare the source and target languages used for constructing prompts of LLMs for translation (\Scref{sec:prompt_lang}) and then compare the LLM translation with the fine-tuned MT and the Google translate system in terms of automatic evaluation metrics (\Scref{sec:auto_eval}). Next, we conduct a fine-grained human evaluation of the different prompting strategies (\Scref{sec:prompt_strategies}). Finally, we show the breakdown results of the best LLM translation strategy on our cultural parallel dataset in terms of cultural regions (\Scref{sec:regions}) and categories (\Scref{sec:categories}). 
% \subsection{Impacts of Prompting Languages}
% \label{sec:prompt_lang}
% % \input{tables/03_external_knowledge_translation}
% % \input{tables/02_language_prompting}
% % \begin{figure}[]
% %     \centering
% %     \includegraphics[width=\columnwidth]{figures/human-evaluation-languages.pdf}
% %     \caption{Source vs target (En vs Zh) language prompts}
% %     \label{fig:language_prompting}
% % \end{figure}
% %We first evaluate the choice of languages used for prompting as this is the first step before examing different prompting strategies. 
% % Figure~\ref{fig:language_prompting} shows the fine-grained human evaluation of the basic instruction and external knowledge prompting strategies using the source and target languages to construct the prompts. 
% % We find that using the target language is consistently better than the source language for constructing prompts in LLM translation performance. 
% % This is further validated by the automatic evaluation in Table~\ref{tab:autoeval_prompting_languages}. 

% As LLMs have been pre-trained on massive texts in multiple languages, their capability of interpreting instructions in different languages has not been comprehensively studied for machine translation. We hypothesize that the language used in the prompt has an impact on the language model's understanding of the instructions and the demonstrations. To investigate the impact of prompt languages on translation, we compare Chinese and English used for writing prompts in six different prompting methods for two translation tasks. The results, shown in Table \ref{tab:autoeval_prompting_languages}, indicate that using Chinese prompts on our dataset is more likely to yield favorable translation outcomes than English prompts. This is evidenced by both traditional translation metrics and our proposed metric for measuring CSI translation accuracy, where Chinese prompts achieve superior performance in terms of CSI-Match scores in 4 out of 6 prompting methods.
% Therefore, we stick to the target language for constructing prompts in the following experiments. 

% From the translation results of SE and CE, we find that SE performs comparably to CE in the EN-ZH task but worse in the ZH-EN task. This is probably due to ChatGPT's different capability of interpreting different regional entities, which is further discussed in \Scref{sec: region_analysis}. 
% We find that Google Translate obviously outperforms Fine-tuned MT and GPT-3.5 on all metrics with a large margin. However, when further fine-tuned with natural language instructions, ChatGPT with basic instruction prompting significantly improves over GPT-3.5, narrowing the gap with Google Translate or even outperforming Google Translate by 1.9 COMET points when using Chinese prompts for EN-ZH translation.
%We observe several findings. First, Google Translate clearly outperforms mBART and GPT-3.5 on all metrics with a large margin. However, when further fine-tuned with natural language instructions, ChatGPT with basic instruction prompting significantly improves over GPT-3.5, narrowing the gap with Google Translate or even outperforming Google Translate by 1.8 COMET points. %However, when it comes to the COMET metric, ChatGPT demonstrates better performance than the rest of the methods.
% The results indicate that the model itself does not show significant awareness of cultural differences. It is worth mentioning that SR performs better than SE and SC on traditional translation metrics, indicating that the quality of LLM translation outputs varies over different runs of sampling, and reranking these outputs is likely to improve corpus-level evaluation metrics. However, SR's performance in CSI-match remains similar to BI, suggesting that LLM is not prone to rank outputs with better cultural entity translation higher than the others.%cultural awareness cues in the prompt when sampling multiple outputs.
% We find that SE, SC, and SR all fail to improve over BI. 
% This indicates that ChatGPT itself lacks accurate internal knowledge of low-frequency CSIs and still struggles with understanding the cultural nuances even with the complex prompting strategies examined in this study.

% Next, we explore the impact of external knowledge on translation accuracy, and the corresponding results can be found in Table \ref{tab:autoeval_prompting_languages}. The findings reveal that both CI and CE outperform BI in all automatic metrics for the target language. This suggests that leveraging external knowledge in the target language can provide additional information to enhance the accuracy of CSI translation.

% Lastly, we compare prompting strategies eliciting LLMs’ internal knowledge (i.e., SE, SC, SR). We find that SE, SC, and SR all fail to improve over BI on traditional machine translation metrics (i.e., BLEU, BLEURT, COMET). But they show an improvement on the CSI-Match score, which indicates that ChatGPT itself has internal knowledge of low-frequency CSIs and has the capacity of understanding the cultural nuances with the complex prompting strategies examined in this study.
% \binwei{TODO: further analysis}. 

% \junjie{\binwei{DONE}Write the findings from the table}


% \junjie{Correlation of human eval to auto eval. Can auto eval on entity accuracy be a proxy to human eval?}
% To further provide a fine-grained assessment of the translation quality regarding cultural-relevant concepts, we conduct a human evaluation of LLM translation with different prompting strategies and traditional NMT systems (\Scref{sec:prompt_strategies}). Finally, we show the breakdown results of the best LLM translation strategy on our cultural parallel dataset in terms of cultural regions (\Scref{sec:regions}). Each part is described in detail below.
% \subsection{Human Evaluation on Prompt Strategies}
% \begin{figure*}[ht!]
%     \centering
%     % \vspace{-3mm}
%     \includegraphics[width=0.88\textwidth]{figures/long-human-evaluation.pdf}
%     \caption{Overall Human Evaluation} %\junjie{Re-draw the figure by increasing the font size. And still keep the figure in one column. Alternatively, you could also reduce the y-axis height to make the figure fit in two columns but not occupy a lot of space.}}
%     \label{fig:human_evaluation}
%     \vspace{-5mm}
% \end{figure*}
% \label{sec:prompt_strategies}

% The overview of human evaluation of MT systems on EN-ZH task by Chinese prompts is shown in Figure \ref{fig:human_evaluation}. In general, we observe the consistent performance differences among MT systems between human and automatic evaluation (e.g., LLM with the CT prompts achieved the best translation performance in \Scref{sec:auto_eval}). Further looking into the different levels of translation quality, we find that external prompting strategies (i.e., CT and CE) significantly outperform Google Translate in translating CSIs, although their performances on traditional automatic evaluation metrics (i.e., BLEU, BLEURT, COMET) are similar.
% %In addition to the automatic evaluation, we show the results of the fine-grained human evaluation in Figure \ref{fig:human_evaluation}. The results of human evaluation validate the conclusions drawn in the automatic evaluation (\Scref{sec:auto_eval}). Additionally, external prompting strategies (i.e., CT and CE) significantly outperform Google Translate in translating CSIs, although their performances on traditional automatic evaluation metrics (i.e., BLEU, BLEURT, COMET) are closed.
% % \par

% % Some examples are shown in Table \ref{tab: Prompting Strategy}.
% To examine the correlation between automatic metrics and human evaluation metrics, we compute the coefficients between automatic metrics and human-annotated CSI translation accuracy, which is obtained by subtracting the number of wrong samples from the sum. Table \ref{tab: correlation} demonstrates that CSI-Match exhibits the strongest relationship with the human judgment on CSI translation quality, indicating its potential as an automatic metric for evaluating CSI accuracy.

==> sections/05_results_old2.tex <==
\section{Results and Analysis}
\label{sec:results}
% To investigate the cultural-awareness of NMT and LLM-based MT, we conduct automatic evaluations between LLM-based MT and popular NMT systems (\Scref{sec:auto_eval}) on six language pair translations. Diving into LLM-based MT, to explore the influence of prompting strategy on LLMs in cultural-specific translation, we conduct automatic evaluations of LLM prompting strategies for English-Chinese translation (\Scref{sec:prompting_auto_eval}). Additionally, to  3) human evaluation on a subset of English-to-Chinese translation(\Scref{sec:human_evaluation}).
In this section, we first compare the cultural awareness of LLM-based MT systems with that of popular NMT systems (\Scref{sec:auto_eval}). Secondly, we compare four prompting strategies of LLM-based MT systems to explore how different prompts affect the LLMs' cultural awareness (\Scref{sec:prompting_auto_eval}). Lastly, we conduct the human evaluation to verify the correlation between automatic evaluation metrics and human assessment (\Scref{sec:human_evaluation}).
\subsection{Which one is better at CSI translation? LLM-based MT or NMT}
\label{sec:auto_eval}
To compare the cultural awareness of large language model-based machine translation (MT) systems with that of neural machine translation (NMT) systems, we employ automatic metrics to evaluate four MT systems: the traditional NMT systems NLLB and Google Translate, and the LLM-based MT systems LLaMA2 and GPT-3.5 (zero-shot BI). Furthermore, to investigate whether traditional dictionary-based terminology translation methods can aid in translating culturally specific items (CSIs), we apply the Append and Replace methods (details in \Scref{sec: mt_systems}) to the open-source MT systems NLLB (NLLB-A and NLLB-R) and LLaMA2 (LLaMA2-A and LLaMA2-R), and evaluate their translation quality.
\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
         % \centering
         \includegraphics[width=\textwidth]{figures/csi-match-1.pdf}
         % \includegraphics[width=0.42\textwidth]{figures/csi-match-2.pdf}
         \caption{Traditional NMT Systems}
         \label{fig:nmt csi-match}
         % \vspace{-3mm}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/csi-match-2.pdf}
         \caption{LLM-based MT Systems}
         \label{fig:llm csi-match}
         % \vspace{-3mm}
     \end{subfigure}
    \caption{CSI-Match Results on Six Language Pairs: The coordinate scale range is [40,100]}
    \label{fig:cs-match-languages}
    \vspace{-3mm}
\end{figure}
\paragraph{NMTs have better accuracy across languages, while LLM-MT better at leveraging external knowledge.}We show accuracy evaluation results of CSI-Match in Figure \ref{fig:cs-match-languages}. For clarity, we demonstrate results of NMT systems (Figure \ref{fig:nmt csi-match}) and LLM-based MT systems (Figure \ref{fig:llm csi-match}) respectively. Notably, NMTs' performances across different languages are generally more consistent compared to LLM-based MTs. Specifically, NLLB and Google Translate perform better in non-Latin languages such as Chinese, Hindi, Tamil, and Telugu when compared to LLaMA2 and GPT-3.5. It is notable that for low-resource languages such as Tamil and Telugu, the performance of LLM-MTs remains limited, and they cannot be considered efficient translation tools. Moreover, we find that straightforward strategies using dictionaries of CSIs, such as Replace (the \textcolor[HTML]{2ca02c}{green} solid line) and Append (the \textcolor[HTML]{ff7f0e}{orange} solid line), are effective on metrics that rely on string-matching, such as CSI-Match, as well as other semantic matching metrics detailed in Appendix \Scref{sec:overall_auto_metric}. However, the appending strategy significantly benefits LLaMA more than NLLB. This suggests that LLaMA's capacity for in-context learning and instruction-following enables the flexible integration of cultural knowledge at test time, a capability not present in traditional NMT systems like NLLB.
% Additionally, we measure the CSI-Match of ChatGPT using basic instructions (BI), and Google Translate (the \textcolor[HTML]{d62728}{red} solid line). We find that Google Translate's performance across different languages is generally more consistent compared to ChatGPT. Specifically, Google Translate performs better in non-Latin languages such as Chinese, Hindi, Tamil, and Telugu, when compared to ChatGPT.
\input{tables/13_understandability}
\input{tables/14_understandablity_prompting}
\input{tables/17_prompting_result_examples}
\paragraph{Understandability Gap of Non-translation CSIs.} Given the cost of evaluation by GPT-4o, we focus on only English-Chinese in two translation directions when evaluating UWR.
Table \ref{tab: Understandability by GPT-4} presents the UWR (Understandability Win Rate) assessed by GPT-4o for various MT systems' output sentences compared to the reference sentences. In addition to UWR across the entire dataset, we show win rates of samples containing complex source items (CSIs) with no translations (\textbf{NT-UWR}). The results indicate that traditional terminology translation methods, such as Appending and Replacing, are able to improve the UWR across the entire dataset. However, they still encounter challenges in improving the comprehensibility of translations that contain CSIs without a well-established reference. Notably, GPT-3.5 performs better than any other MT systems on NT-UWR, which potentially suggests that the instruction-tuning of LLMs beyond the translation task may be beneficial for the model to generate explanation-based translations for these non-translation CSIs.

\subsection{Prompting Strategy Evaluation}
\label{sec:prompting_auto_eval}
As LLM-based MTs open up the opportunity to incorporate free-form external knowledge for improving the understandability of non-translation CSIs, we explore various prompting strategies by incorporating additional cultural information alongside dictionaries to improve translation. We compare different prompting strategies on English-Chinese translations. 
% We examine 2-shot approaches to obtain results from GPT-3.5 and LLaMA2. Especially for complex prompting strategies including CE, SE, and SR, we use 2-shot examples that are tailored for culturally-aware translation.
Table~\ref{tab:understandablity_prompting_methods} shows the evaluation results of different prompting methods.

\paragraph{External Cultural Knowledge Enhances CSI Translation Quality of LLM-MTs.} Comparing the strategies of using external knowledge in prompts (i.e., CT and CE), we observe that LLMs can effectively leverage both direct translations and indirect descriptions. Specifically, CT greatly enhances the CSI-Match score for CSI translation. However, CT only offers limited improvement in GPT-3.5's UWR because CT often generates results identical to the reference. For example, $54.8\%$ of CT outputs are the same as references when translating from Chinese to English. More importantly, 2-shot CE significantly improves NT-UWR from $31.7$ to $41.3$ in English to Chinese translations. This suggests that CSI explanations offer significant assistance in translating CSIs, particularly those without well-known translations. CE fails to improve NT-UWR for Chinese-to-English translations because we use English explanations for CSIs, and no-translation CSIs from Chinese to English lack explanations in English. In Table \ref{tab: Prompting Strategy Examples}, we quantitatively show output examples of "Polenta," an Italian corn porridge. Interestingly, its Chinese translation on Wikidata is merely a transliteration. Under the CT strategy, GPT-3.5 directly copies this transliteration into the output, which may be considered correct yet not comprehensible for native speakers of the target language. In contrast, GPT-3.5 using CE integrates an explanation into the translation, describing the term as "corn porridge" in Chinese. This translation makes it much easier for readers to understand the nature of Polenta.

\paragraph{Internal Cultural Knowledge Benefits CSI translation of LLM-MTs} We use SE to elicit LLMs’ internal knowledge and find that 2-shot SE of GPT-3.5 improves translation performance on all metrics for both English-to-Chinese and Chinese-to-English translations. Notably, SE improves NT-UWR for Chinese-to-English translations by generating explanations for these CSIs which are typically unique to the target-language culture, and then translating the sentences based on those explanations. This suggests that GPT-3.5 itself might already possess a certain amount of cultural knowledge of CSIs. In Table \ref{tab: Prompting Strategy Examples}, SE successfully generates an explanation for "polenta" and incorporates this explanation into the translation as "corn porridge", which is easy to be understood by Chinese native speakers. More generation examples are in Appendix \Scref{sec:expr_examples}.
% On the other hand, SR proves beneficial on ChatGPT for CSI-Match but does not improve the understandability of CSI translations, indicating that LLMs inherently possess internal knowledge of low-frequency CSIs but still can not capture cultural nuances through the SR prompting strategy examined in this study. 
% In Table~\ref{tab: Prompting Strategy Examples}, 2-shot SR translates ``Polenta'' as ``cornmeal,'' similar to the baseline (BI). However, SE successfully translates it into ``corn porridge.'' This suggests that ChatGPT possesses background knowledge of Polenta but struggles to spontaneously elicit it to generate and select the most understandable translations.
% \junjie{SE is 2-shot, but SR here is zero-shot? The last sentence is not fair.}
\subsection{Human Evaluation}
\label{sec:human_evaluation}
\input{tables/19_metric_consistency_all}
To compare the consistency between automatic metrics and human evaluation, we conduct a human evaluation on a subset of 200 English-to-Chinese translations. We assess the outputs from eight MT systems: NLLB, LLaMA2, Google Translate, and GPT-3.5 across zero-shot BI, two-shot BI, CT, CE, and SE settings. A native Chinese speaker evaluates the accuracy and usability, readability, and UWR of the outputs. We then calculate Pearson's correlation coefficients between automatic evaluation metrics and human assessments of accuracy and UWR. Specifically, we compare the performance of CSI-Match and UWR with four traditional automatic evaluation metrics: BLEU, BLEURT, COMET, and Exact-Match. The results, presented in Table \ref{tab: correlation}, indicate that CSI-Match exhibits the highest correlation with human accuracy, while UWR shows the highest correlation with human UWR. These findings suggest that CSI-Match and UWR are effective evaluation metrics for assessing the translation of CSIs, which can better capture cultural nuances.
% \paragraph{CSI-Match and Human Evaluation Accuracy Are Consistent.}  we also calculate the correlation between automatic evaluation metrics and human evaluation, where we consider the translation correct in human evaluation if the translation is categorized into all the translation strategies except Copy and Wrong.  CSI-Match has the highest correlation score at 94.7 with human evaluation, suggesting that CSI-Match can be an efficient evaluation metric for CSIs with a reference translation. 

% \paragraph{GPT-4 and Human Evaluation Are Consistent.}
% Table \ref{tab: correlation} shows the Overall-U evaluated by both GPT-4 and human annotators. Specifically, we randomly select 200 samples from the English-to-Chinese translation dataset and have human annotators evaluate the understandability of output translations by the four different methods. The results indicate a high level of consistency between human annotations and GPT-4's evaluations.


==> tables/01_examples.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{llll}
    \toprule
    % \textbf{Source} & \multicolumn{2}{l}{alongside other Italian pastries \& cannoli like \textbf{cannoli} and \textbf{sfogliatelle} }\\
    % \textbf{Reference} & \multicolumn{2}{l}{alongside other Italian pastries \junjie{Replace this to human translation}}\\ 
    % \midrule \midrule
    \textbf{Strategy}     &  \textbf{Prompt}  & \textbf{Target Outputs}\\
    \midrule
\multirow{3}{*}{Basic Instruction (\textbf{BI})} & {Translate the following English text to Chinese}& \begin{CJK}{UTF8}{gbsn}..., 与其他意大利点心比如{\color{blue}卡诺利} \end{CJK}\\
&&\begin{CJK}{UTF8}{gbsn}{\color{blue}(\textit{transliteration of cannoli}), 斯福利雅}\end{CJK} \\
&&\begin{CJK}{UTF8}{gbsn}{\color{blue}蒂 (\textit{ transliteration of sfogliatelle})}一起\end{CJK}\\
\midrule

\multirow{3}{*}{CSI Translation (\textbf{CT})} & The Chinese translation of culture entities in the sentence is as following:& \begin{CJK}{UTF8}{gbsn}...，以及{\color{blue}里考塔芝士卷 (\textit{Ricotta cheese rolls})}\end{CJK}\\
& {\color{blue}{\textit{cannoli:\begin{CJK}{UTF8}{gbsn}里考塔芝士卷(\textit{Ricotta cheese rolls}), 奶油甜馅煎饼卷 (\textit{Sweet Cream pancake rolls})\end{CJK}}}}& \begin{CJK}{UTF8}{gbsn}和{\color{blue}意大利翻糖酥饼 (\textit{Italian fondant shortbread})}\end{CJK}\\
&Translate the following English text to Chinese & \begin{CJK}{UTF8}{gbsn}等其他意大利糕点一道供应。\end{CJK}\\
\midrule

\multirow{3}{*}{CSI Explanation (\textbf{CE})} & {The explanation of culture entities in the sentence is as following:} &\begin{CJK}{UTF8}{gbsn}..., 与糕点如{\color{blue}cannoli}和{\color{blue}sfogliatelle}等其他\end{CJK}\\
&{\color{blue}{\textit{Cannoli are Italian pastries consisting of tube-shaped shells of fried pastry dough ...}}} &  \begin{CJK}{UTF8}{gbsn}意大利糕点一同供应\end{CJK}\\
&Translate the following English text to Chinese &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
\midrule

\multirow{4}{*}{Self-Explanation (\textbf{SE})} & User: Please explain cannoli in {\color{blue}{[Source Sentence]}} &\begin{CJK}{UTF8}{gbsn}..., 与糕点如{\color{blue}cannoli}和{\color{blue}sfogliatelle}等其他\end{CJK}\\
&LLM: {\color{blue}{[Explanation]}}&  \begin{CJK}{UTF8}{gbsn}意大利糕点一起\end{CJK}\\
&User: According to your explanations to cannoli, only &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
&translate the following English text to Chinese&\\
\midrule


% \multirow{5}{*}{Self-Correction (\textbf{SC})} & {User: Translate the following English text to Chinese: {\color{blue}{[Source Sentence]}}.}& \begin{CJK}{UTF8}{gbsn}和其他意大利糕点，如卡诺利\end{CJK}\\
% &  {\color{blue}{\textit{Please firstly think about how to ensure that the culturally relevant words in the}}} &  \begin{CJK}{UTF8}{gbsn}和卷层蛋糕一起，享用\end{CJK}\\
% & {\color{blue}{\textit{sentence are translated into Chinese words that Chinese readers can understand.}}} & \\
% & LLM: \color{blue}{[Analysis]} & \\
% & User: According to your analysis above, please translate the sentence& \\
% \midrule

\multirow{7}{*}{Self-Ranking (\textbf{SR})} & {User: Translate the following English text to Chinese: {\color{blue}{[Source Sentence]}}.}& \begin{CJK}{UTF8}{gbsn}..., 与{\color{blue}坎诺利卷 (\textit{transliteration of cannoli}) }和\end{CJK}\\
&  {\color{blue}{\textit{Please give [Generated Number] most likely translations, and ensure ''cannoli'' }}} &  \begin{CJK}{UTF8}{gbsn}{\color{blue}意大利糕点 (\textit{An Italian pastry}
)}一起。\end{CJK}\\
& {\color{blue}{\textit{in each result to correspond to different translations}}} & \\
& LLM: \color{blue}{[Translations]} & \\
& User: \color{blue}{\textit{Please select the the best translation result of entities: cannoli.}}& \\
&\color{blue}{\textit{The translation of entitis  in the sentence should be the closest to its explanation, }}& \\
&\color{blue}{\textit{and is easy to be understood by Chinese readers.}}&\\
 \midrule \midrule   
    \textbf{Source} & \multicolumn{2}{l}{They are also commonly available at Italian-American bakeries in the United States,} \\
    & alongside other Italian pastries like {\color{red}{cannoli}} and {\color{red}{sfogliatelle}}.\\
    \textbf{Reference} & \multicolumn{2}{l}{\begin{CJK}{UTF8}{gbsn}在美国,它们通常也可以在意大利裔美国人开的面包店中见到，就像其它意大利糕点\end{CJK}}\\
    &\begin{CJK}{UTF8}{gbsn}比如{\color{red}{里考塔芝士卷 (\textit{Ricotta cheese rolls})}}和{\color{red}{意式千层酥(\textit{Italian mille-feuille})}}一样。 \end{CJK} \\
    
    \bottomrule
    \end{tabular}}
    \caption{Prompting strategy examples (\textbf{Top}) and a source-reference sentence pair for En-Zh translation (\textbf{Bottom})
    % \junjie{\binwei{Done}Confirm the prompts in self-correction and self-ranking}
    }
    \label{tab: Prompting Strategy}
    \vspace{-3mm}
\end{table*}

% \begin{table*}[]
%     \centering
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{llll}
%     \toprule
%     textbf{Source} & alongside other Italian pastries & cannoli like \textbf{cannoli} and \textbf{sfogliatelle} 
%     \textbf{Strategy}     &  \textbf{Prompt} & \textbf{Source} & \textbf{CSI} & \textbf{Target}\\
%     \midrule
% \multirow{2}{*}{Basic Instruction (\textbf{BI})} & {Translate the following English text to Chinese}& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}除了cannoli和sfogliatelle等\end{CJK}\\
% &&  like \textbf{cannoli} and \textbf{sfogliatelle}& sfogliatelle&\begin{CJK}{UTF8}{gbsn}其他意大利糕点之外，还有...\end{CJK}\\
% \midrule

% \multirow{3}{*}{CSI Translation (\textbf{ET})} & {The Chinese translation of the item is as following:}& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}和里考塔芝士卷、\end{CJK}\\
% & {cannoli:\begin{CJK}{UTF8}{gbsn}里考塔芝士卷\end{CJK}}&  like \textbf{cannoli} and \textbf{sfogliatelle} & sfogliatelle &\begin{CJK}{UTF8}{gbsn}意大利千層面酥饼一起端上来\end{CJK}\\
% &Translate the following English text to Chinese& & &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
% \midrule

% \multirow{3}{*}{CSI Explanation (\textbf{CE})} & {The explanation of cannoli is \textit{Cannoli are Italian pastries}}& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}与糕点如cannoli和sfogliatelle\end{CJK}\\
% &\textit{consisting of tube-shaped shells of fried pastry dough ...} &  like \textbf{cannoli} and \textbf{sfogliatelle}& sfogliatelle&\begin{CJK}{UTF8}{gbsn}等其他意大利糕点并置\end{CJK}\\
% &Translate the following English text to Chinese& & &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
% \midrule

% \multirow{4}{*}{Self-Explanation (\textbf{SE})} & {User: Please explain cannoli in [Source Sentence]}& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}除了義式酥皮卷和sfogliatelle等\end{CJK}\\
% &LLM: [Explanation]&  like \textbf{cannoli} and \textbf{sfogliatelle}& sfogliatelle&\begin{CJK}{UTF8}{gbsn}其他意大利糕點外，\end{CJK}\\
% &User: According to your understanding to cannoli, only &&&\begin{CJK}{UTF8}{gbsn}Cannoli是傳統的意大利糕點之一。\end{CJK}\\
% &translate the following English text to Chinese: [Source Sentence]&&&\\
% \midrule


% \multirow{2}{*}{Self-Correction (\textbf{SC})} & {Translate the following }& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}除了cannoli和sfogliatelle等\end{CJK}\\

% &English text to Chinese&  like \textbf{cannoli} and \textbf{sfogliatelle}& sfogliatelle&\begin{CJK}{UTF8}{gbsn}其他意大利糕点之外，还有...\end{CJK}\\
% \midrule

% \multirow{2}{*}{Self-Ranking (\textbf{SR})} & {Translate the following }& alongside other Italian pastries & cannoli &\begin{CJK}{UTF8}{gbsn}除了cannoli和sfogliatelle等\end{CJK}\\

% &English text to Chinese&  like \textbf{cannoli} and \textbf{sfogliatelle}& sfogliatelle&\begin{CJK}{UTF8}{gbsn}其他意大利糕点之外，还有...\end{CJK}\\

%     \bottomrule
%     \end{tabular}}
%     \caption{Prompting Strategy Examples}
%     \label{tab: Prompting Strategy}
% \end{table*}

==> tables/02_auto_evaluation.tex <==
% \begin{table}[]
%     \centering
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Method}     &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
%     \midrule
%      mBART               &15.0          &0.441         & 67.9         & 20.9  \\
%      text-davinci-003    &22.2          &0.482         & 72.0         & 25.0  \\
%      ChatGPT             &27.2          &0.547         &\textbf{78.6} & 28.5 \\
%      Google              &\textbf{29.3} &\textbf{0.561} & 77.1         & \textbf{32.6}  \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Results of Basic Translation Methods}
%     \label{tab: Basic Translation Methods}
% \end{table}

\begin{table}[]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method}     &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
    \midrule
     mBART               &15.0          &0.441         & 67.9         & 12.0  \\
     Google              &\textbf{32.2} & \textbf{0.561} & \textbf{77.1}         & \textbf{16.3}  \\
     GPT-3.5    &21.6          &0.482         & 72.0         & 12.1  \\
     % ChatGPT             &27.2          &0.547         &\textbf{78.6} & 28.5 \\
     \midrule
     \textbf{ChatGPT(BI)} & 26.2 & 0.550 & 78.9 & 29.1 \\
     \textbf{CT}  & \textbf{28.7} & \textbf{0.569} & \textbf{79.5} & \textbf{37.5} \\
     \textbf{CE}  & 26.8 & 0.554 & 77.8 & 32.7 \\
     \textbf{SE}  & 21.2          &0.542         &75.3 & 26.3 \\
     \textbf{SC}  &23.7          &0.540         &76.6 & 30.2 \\
     \textbf{SR}  &19.3          &0.490         &70.8 & 29.4 \\
    \bottomrule
    \end{tabular}}
    \caption{Automatic evaluation on basic MT methods (\textbf{Up)} and prompt-based LLM translation (\textbf{Bottom}).}
    \label{tab: Basic Translation Methods}
\end{table}

==> tables/02_chinese_auto_evaluation.tex <==

\begin{table*}[h!]
    \centering
    \vspace{-4mm}
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{l|rrrr|rrrr}
    \toprule
    \textbf{Method}  & \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}  & \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
    \midrule
    &  \multicolumn{4}{c|}{EN-ZH}&\multicolumn{4}{c}{ZH-EN}\\
    
    \textbf{NLLB} & 23.2 & 0.558 & 77.0 & 53.1 & 27.0 & 0.594 & 76.5 & 68.7 \\
    \textbf{NLLB-A} & 17.3 & 0.447 & 62.8 & 62.0 & 22.1 & 0.510 & 65.9 &68.5\\
    \textbf{NLLB-R} & 26.3	& 0.551 & 76.8 & \textbf{83.2} & 31.5 & 0.633 & 78.5 & \textbf{97.4} \\
    \textbf{LLaMA2} & 17.1 & 0.529 & 75.8 & 45.0 & 26.1 & 0.595 & 77.9 & 70.9\\
    \textbf{LLaMA2-A} & 18.3 &	0.518 & 74.4 & 80.2 & 29.1 & 0.629 & 79.0 & 85.6 \\
    \textbf{LLaMA2-R} & 19.2 & 0.547 & 76.8 & 78.1 & 27.7 & 0.618 & 78.9 & 80.6 \\
    \textbf{ChatGPT}  & 29.3 &	0.642 & 82.9 & 67.2 & 32.5 & 0.668 & 80.9 &77.7\\
    \textbf{Google} & 38.3	& 0.679 & 84.2 & 71.9 & 41.1 & 0.697 & 82.2 &79.5\\
    \bottomrule
    \end{tabular}
    }
    \caption{Automatic evaluation of all MT methods on six language pairs from both translation directions.\binwei{Add ChatGPT-A and ChatGPT-R} and add a figure of other languages}
    \label{tab:autoeval_chinese}
    % \vspace{-5mm}
\end{table*}
  


==> tables/02_language_prompting.tex <==
\begin{table}[!h]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method}    & \textbf{Lang.} &  \textbf{Correct} & \textbf{Copy} & \textbf{Understandable} & \textbf{Wrong}\\
    \midrule
    \multirow{2}{*}{Basic Instruction} & En & 44 & 18 & 7 & 35 \\
    &Zh  & 60 & 20 & 5 & 19 \\
    \multirow{2}{*}{CSI Translation} & En   & 76 & 7  & 3 & 18 \\
       & Zh   & 88 & 6  & 4 & 6 \\
    \multirow{2}{*}{CSI Explanation} & En   & 55 & 23 & 14 & 12 \\
    & Zh   & 64 & 18 & 12 & 10 \\
    \bottomrule
    \end{tabular}}
    \caption{Source vs target (En vs Zh) language prompts}
    \label{tab:humaneval_prompt_language}
\end{table}


==> tables/03_evaluation_prompting.tex <==
\begin{table*}[h!]
    \centering
    % \vspace{-3mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccc}
    \toprule
    \multirow{1}{*}{\textbf{Method}}     &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match} & \textbf{Overall-U} & \textbf{NT-U} &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match} & \textbf{Overall-U} & \textbf{NT-U}\\
    \midrule
    &\multicolumn{6}{c|}{ChatGPT}&\multicolumn{6}{c}{LLaMA2-7B}\\
    \textbf{BI} & 29.3 & 0.642 & 82.9 & 67.2 & && 14.8 & 0.503 & 73.6 & 35.1 && \\
    \textbf{CT} & \textbf{30.6} & 0.646 & \textbf{83.1} & \textbf{84.0} & & & \textbf{16.6} & \textbf{0.520} & 73.3 & \textbf{70.3} \\
    \textbf{CE} & 29.0 & \textbf{0.647} & \textbf{83.1} & 66.6 & & & 10.5 & 0.463 &69.3 & 35.5 \\
    \textbf{SE} & 27.9 & 0.638 & 82.8 & 65.1 & & & 14.3 & 0.509 & \textbf{73.7} & 35.1\\
    % \textbf{SC} & 28.9 & 0.636 & 82.0 & 67.3 & 11.8 & 0.512 & 73.2 & 34.9\\
    \textbf{SR} & 29.3 & 0.642 & 82.8 & 69.2 & && 10.4 & 0.497 & 72.1 & 37.9\\
    \bottomrule
    \end{tabular}
    }
    \caption{Automatic evaluation of MT methods on English-Chinese translations. \binwei{add 2-shot chatgpt and 0-shot llama}}
    \label{tab:autoeval_prompting_methods}
     \vspace{-5mm}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|lcccc|cccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Task}}&
%     \multirow{2}{*}{\textbf{Method}}     &  \multicolumn{4}{c|}{\textbf{Source Language (En)}}&\multicolumn{4}{c}{\textbf{Target Language (Zh)}}\\
%     && \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}  &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
%     \midrule
%     % &\multicolumn{4}{c|}{EN}&\multicolumn{4}{c}{ZH}\\
%     % \cmidrule{2-9}
    
%     \multirow{3}{*}{\textbf{EN-ZH}} &\textbf{ChatGPT(BI)} & \textbf{28.7} & 0.547  & 76.6 & 13.6 & 26.2 & \textbf{0.550} & \textbf{78.9} & \textbf{15.4} \\
%     &\textbf{CT}  & 27.6 &  0.553 & 76.0 & 37.5 & \textbf{28.7} & \textbf{0.569} & \textbf{79.5} & \textbf{37.5}\\
%     &\textbf{CE}           & 13.9 & 0.551 & 75.9 & 30.1 & \textbf{26.8} & \textbf{0.554} & \textbf{77.8} & \textbf{32.7}   \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Automatic evaluation of prompting strategies in the source and target languages}
%     \label{tab:autoeval_prompting_languages}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|l|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Task}}&
%     \multirow{2}{*}{\textbf{Method}}     &  \multicolumn{4}{c|}{\textbf{Source Language}}&\multicolumn{4}{c}{\textbf{Target Language}}\\
%     && \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}  &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
%     \midrule
%     % &\multicolumn{4}{c|}{EN}&\multicolumn{4}{c}{ZH}\\
%     % \cmidrule{2-9}
    
%     \multirow{6}{*}{\textbf{EN-ZH}} &\textbf{Google} &\textbf{32.2} & \textbf{0.561} & \textbf{77.1} & \textbf{16.3} & - & - & - & - \\ &\textbf{ChatGPT(BI)} & \textbf{28.7} & 0.547  & 76.6 & 13.6 & 26.2 & \textbf{0.550} & \textbf{78.9} & \textbf{15.4} \\
%     &\textbf{CT}  & 27.6 &  0.553 & 76.0 & 37.5 & \textbf{28.7} & \textbf{0.569} & \textbf{79.5} & \textbf{37.5}\\
%     &\textbf{CE}           & 13.9 & 0.551 & 75.9 & 30.1 & \textbf{26.8} & \textbf{0.554} & \textbf{77.8} & \textbf{32.7}   \\
%     &\textbf{SE} & - & -  & - & - & 21.2          &0.542         &75.3 & 26.3\\
%     &\textbf{SC}   & - & -  & - & - &23.7          &0.540         &76.6 & 30.2 \\
%     &\textbf{SR}    & - & -  & - & - &19.3          &0.490         &70.8 & 29.4 \\
%     % \midrule
%     % \multirow{6}{*}{\textbf{ZH-EN}} &\textbf{ChatGPT(BI)} & \textbf{28.7} & 0.547  & 76.6 & 13.6 & 26.2 & \textbf{0.550} & \textbf{78.9} & \textbf{15.4} \\
%     % &\textbf{CT}  & 27.6 &  0.553 & 76.0 & 37.5 & \textbf{28.7} & \textbf{0.569} & \textbf{79.5} & \textbf{37.5}\\
%     % &\textbf{CE}           & 13.9 & 0.551 & 75.9 & 30.1 & \textbf{26.8} & \textbf{0.554} & \textbf{77.8} & \textbf{32.7}   \\
%     % &\textbf{SE} & - & -  & - & - & 21.2          &0.542         &75.3 & 26.3\\
%     % &\textbf{SC}   & - & -  & - & - &23.7          &0.540         &76.6 & 30.2 \\
%     % &\textbf{SR}    & - & -  & - & - &19.3          &0.490         &70.8 & 29.4 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{\binwei{Old}Automatic evaluation of prompting strategies in the source and target languages}
%     \label{tab:autoeval_prompting_languages}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|l|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Task}}&
%     \multirow{2}{*}{\textbf{Method}}     &  \multicolumn{4}{c|}{\textbf{EN Prompts}}&\multicolumn{4}{c}{\textbf{ZH Prompts}}\\
%     && \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}  &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
%     \midrule
%     % &\multicolumn{4}{c|}{EN}&\multicolumn{4}{c}{ZH}\\
%     % \cmidrule{2-9}
    
%     \multirow{9}{*}{\textbf{EN-ZH}} &\textbf{OPUS-MT} & 19.4 & 0.458 & 68.7  & 52.7 & - & - & - & - \\
%     &\textbf{Google} & \textbf{33.2} & 0.547  & 76.6 & 67.1 & - & - & - & - \\
%     &\textbf{GPT3.5} & 23.9 & 0.515  & 74.9 & 58.5 & 23.5$\reddownarrow$ & 0.534$\greenuparrow$ & 76.2$\greenuparrow$ & 60.7$\greenuparrow$ \\
%     &\textbf{BI} & 26.3 & 0.541  & 76.3 & 64.7 & 26.8$\greenuparrow$ & 0.551$\greenuparrow$ & 77.6$\greenuparrow$ & 63.9$\reddownarrow$ \\
%     &\textbf{CT}  & 28.6 &  \textbf{0.558}  & \textbf{77.6} &  \textbf{87.1} &  \textbf{28.3}$\reddownarrow$ &  \textbf{0.561}$\greenuparrow$ &  \textbf{78.1}$\greenuparrow$ & \textbf{86.6}$\reddownarrow$ \\
%     &\textbf{CE} & 23.5 & 0.546  & 76.7 & 66.5 &23.5 & 0.553$\greenuparrow$ & 77.3$\greenuparrow$ & 67.7$\greenuparrow$  \\
%     &\textbf{SE} & 25.2 & 0.546  & 76.6 & 65.3 & 24.8$\reddownarrow$ & 0.547$\greenuparrow$ & 76.5$\reddownarrow$ & 69.0$\greenuparrow$  \\
%     &\textbf{SC}  & 25.3 &  0.538 & 75.0  & 64.3 & 25.6$\greenuparrow$ & 0.556$\greenuparrow$ & 77.7$\greenuparrow$  &66.1$\greenuparrow$ \\
%     &\textbf{SR}    & 27.5 & 0.544  & 76.8 & 65.0 & 27.3$\reddownarrow$ & 0.551$\greenuparrow$ & 77.6$\greenuparrow$ & 65.1$
%     \greenuparrow$ \\
%     \midrule
%     \multirow{9}{*}{\textbf{ZH-EN}}&\textbf{OPUS-MT}& - & - & - & - & 15.1 & 0.512  & 70.2 & 71.1  \\
%     &\textbf{Google} & - & - & - & - & \textbf{26.7} & 0.595  & 76.6 & 84.0  \\
%     &\textbf{GPT3.5}& 18.8 & 0.556 & 74.5 & 79.9 & 19.0$\greenuparrow$ & 0.560$\greenuparrow$  & 74.4$\reddownarrow$& 79.1$\reddownarrow$  \\
%     &\textbf{BI} & 20.2 & 0.572  & 75.0 & 80.6 &22.0$\greenuparrow$ & 0.580$\greenuparrow$  & 75.9$\greenuparrow$ & 81.3$\greenuparrow$ \\
%     &\textbf{CT} & 19.0 & \textbf{0.592} & \textbf{76.0} & \textbf{94.7}  & 22.5$\greenuparrow$ & \textbf{0.599}$\greenuparrow$  & \textbf{76.7}$\greenuparrow$&\textbf{95.3$\greenuparrow$}\\
%     &\textbf{CE}  & 20.6 & 0.589 & 75.9 & 89.7 & 20.2$\reddownarrow$ & 0.588$\reddownarrow$  & 76.1$\greenuparrow$ & 88.4$\reddownarrow$ \\
%     &\textbf{SE} & 18.8 & 0.578 & 74.8 & 80.2 & 19.4$\greenuparrow$ & 0.570$\reddownarrow$  & 75.6$\greenuparrow$ & 82.3$\greenuparrow$  \\
%     &\textbf{SC} & 18.7 & 0.564& 73.9 & 81.7   & 19.8$\greenuparrow$ & 0.575$\greenuparrow$  & 75.2$\greenuparrow$ & 82.5$\greenuparrow$\\
%     &\textbf{SR} & 20.1& 0.577& 75.7 & 80.5   & 22.1$\greenuparrow$ & 0.584$\greenuparrow$  & 76.3$\greenuparrow$ & 82.2$\greenuparrow$ \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Automatic evaluation of MT methods on English-Chinese and Chinese-English translations. Six different prompting strategies (\textbf{BI}, \textbf{CT}, \textbf{CE}, \textbf{SE}, \textbf{SC}, \textbf{SR}) are performed on ChatGPT. $\greenuparrow/\reddownarrow$ indicates a better/worse performance when using Chinese prompts against English prompts.}
%     \label{tab:autoeval_prompting_languages}
%     % \vspace{-3mm}
% \end{table*}

==> tables/04_CoT_translation.tex <==
\begin{table}[]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method}     &  \textbf{BLEU} & \textbf{BLEURT} & \textbf{COMET} & \textbf{CSI-Match}\\
    \midrule
     \textbf{BI}             &\textbf{26.2}          &\textbf{0.550}        &\textbf{78.9} & - \\
     \textbf{SE}              &21.2          &0.542         &75.3 & - \\
     \textbf{SC}               &23.7          &0.540         &76.6 & - \\
     \textbf{SR}                  &19.3          &0.490         &70.8 & - \\
    \bottomrule
    \end{tabular}}
    \caption{CoT Translation Methods}
    \label{tab: CoT Translation Methods}
\end{table}

==> tables/05_human_evaluation.tex <==
% \begin{table}[]
%     \centering
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Method}  & \textbf{Correct} & \textbf{Copy} &  \textbf{Understandable} & \textbf{Wrong}\\
%     \midrule
%     mBART                  & 24 & 15 & 9 & 56 \\
%     text-davinci-003       & 19 & 32 & 9 & 44 \\
%     Google                 & 51 & 23 & 5 & 25 \\
%     \midrule
%     Basic Instruction (EN) & 44 & 18 & 7 & 35 \\
%     Basic Instruction (ZH) & 60 & 20 & 5 & 19 \\
%     CSI Translation (EN)   & 76 & 7  & 3 & 18 \\
%     CSI Translation (ZH)   & 88 & 6  & 4 & 6 \\
%     CSI Explanation (EN)   & 55 & 23 & 14 & 12 \\
%     CSI Explanation (ZH)   & 64 & 18 & 12 & 10 \\
%     \midrule
%     Zero-Shot-COT        & 49 & 38 & 10 & 7 \\
%     Self-Correction      & 53 & 8 & 16 & 27 \\
%     Self-Ranking         & 52 & 14 & 14 & 24 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Overall Human Evaluation}
%     \label{tab: Overall Human Evaluation}
% \end{table}

\begin{table}[]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method}  & \textbf{Correct} & \textbf{Copy} &  \textbf{Understandable} & \textbf{Wrong}\\
    \midrule
    mBART                  & 24 & 15 & 9 & 56 \\
    text-davinci-003       & 19 & 32 & 9 & 44 \\
    Google                 & 51 & 23 & 5 & 25 \\
    \midrule
    Basic Instruction  & 60 & 20 & 5 & 19 \\
    CSI Translation    & 88 & 6  & 4 & 6 \\
    CSI Explanation    & 64 & 18 & 12 & 10 \\
    \midrule
    Zero-Shot-COT        & 49 & 38 & 10 & 7 \\
    Self-Correction      & 53 & 8 & 16 & 27 \\
    Self-Ranking         & 52 & 14 & 14 & 24 \\
    \bottomrule
    \end{tabular}}
    \caption{Overall human evaluation.}
    \label{tab: Overall Human Evaluation}
\end{table}

==> tables/06_correlation.tex <==
% \begin{table}[h]
%     \centering
%     \resizebox{0.7\linewidth}{!}{
%     \begin{tabular}{lc}
%     \toprule
%     \textbf{Metrics}  & \textbf{Kendall’s} & \textbf{Pearson’s} \\
%     \midrule
%     BLEU &24.5&44.4\\
%     BLEURT &45.8&44.4\\
%     COMET&54.9&50.0\\
%     CSI-Match&\textbf{81.2}&\textbf{72.2}\\
%     \bottomrule
%     \end{tabular}}
%     \caption{Ranking Coefficients between automatic metrics and human evaluation on CSI translation accuracy}
%     \label{tab: correlation}
%     \vspace{-3mm}
% \end{table}
% \begin{table}
%     \centering
%     \resizebox{0.7\linewidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%     \textbf{Metrics}  & \textbf{Spearman’s} & \textbf{Kendall’s}\\
%     \midrule
%     BLEU &37.7&25.4\\
%     BLEURT &53.8&45.7\\
%     COMET&39.3&31.0\\
%     CSI-Match&\textbf{96.7}&\textbf{88.9}\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Ranking Coefficients between automatic metrics and human evaluation on CSI translation\binwei{TODO:update it by understandability}}
%     \label{tab: correlation}
%     \vspace{-3mm}
% \end{table}

\begin{table}
    \centering
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{lc}
    \toprule
    \textbf{Metrics}  & \textbf{Pearson’s}\\
    \midrule
    BLEU & 88.8 \\
    BLEURT & 90.5 \\
    COMET&89.5\\
    CSI-Match&\textbf{94.7}\\
    \bottomrule
    \end{tabular}
    }
    \caption{Ranking Coefficients between automatic metrics and human evaluation on CSI translation}
    \label{tab: correlation}
    \vspace{-3mm}
\end{table}

==> tables/08_stats_region.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llc}
    \toprule
    \textbf{Region} & \textbf{Countries} & \textbf{Sum} \\
     \midrule
    North America  &  United States of America & 517 \\
    (596)    &  Canada & 49 \\
        &  Mexico & 24 \\
        & Jamaica &  6 \\
    \midrule
    Europe & United Kingdom & 140 \\
    (330)&Italy&76\\
    &France&26\\
    &Germany&24\\
    &Switzerland&23\\
    &  Spain  & 11 \\
        &  Russia & 10 \\
        & Netherlands & 6 \\
        & Belgium & 6 \\
        & Denmark & 4 \\ 
        & Austria & 4 \\
    \midrule
    East\&\&Southeast Asia & Singapore & 59\\
    (176)&Japan&56\\
    &China&45\\
    &Korea&9\\
    &Malaysia&7\\
    \midrule
    Oceania (46) & Australia& 46\\
    \bottomrule
    \end{tabular}}
    \caption{Data Statistics by Regions}
    \label{tab: stats_region}
\end{table}

==> tables/09_quality_analysis.tex <==
\begin{table*}[]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{llll}
    \toprule
    % \textbf{Source} & \multicolumn{2}{l}{alongside other Italian pastries \& cannoli like \textbf{cannoli} and \textbf{sfogliatelle} }\\
    % \textbf{Reference} & \multicolumn{2}{l}{alongside other Italian pastries \junjie{Replace this to human translation}}\\ 
    % \midrule \midrule
    \textbf{Strategy}     &  \textbf{Prompt}  & \textbf{Target Outputs}\\
    \midrule
\multirow{2}{*}{Basic Instruction (\textbf{BI})} & {Translate the following English text to Chinese}& \begin{CJK}{UTF8}{gbsn}除了cannoli和sfogliatelle等\end{CJK}\\
&&\begin{CJK}{UTF8}{gbsn}其他意大利糕点之外，还有...\end{CJK}\\
\midrule

\multirow{3}{*}{CSI Translation (\textbf{CT})} & {The Chinese translation of the item is as following:}& \begin{CJK}{UTF8}{gbsn}和里考塔芝士卷、\end{CJK}\\
& {\color{blue}{\textit{cannoli:\begin{CJK}{UTF8}{gbsn}里考塔芝士卷, 奶油甜馅煎饼卷\end{CJK}}}}& \begin{CJK}{UTF8}{gbsn}意大利千層面酥饼一起端上来\end{CJK}\\
&Translate the following English text to Chinese &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
\midrule

\multirow{3}{*}{CSI Explanation (\textbf{CE})} & {The explanation of cannoli is {\color{blue}{\textit{Cannoli are Italian pastries}}}} &\begin{CJK}{UTF8}{gbsn}与糕点如cannoli和sfogliatelle\end{CJK}\\
&{\color{blue}{\textit{consisting of tube-shaped shells of fried pastry dough ...}}} &  \begin{CJK}{UTF8}{gbsn}等其他意大利糕点并置\end{CJK}\\
&Translate the following English text to Chinese &\begin{CJK}{UTF8}{gbsn}\end{CJK}\\
\midrule

\multirow{4}{*}{Self-Explanation (\textbf{SE})} & User: Please explain cannoli in {\color{blue}{[Source Sentence]}} &\begin{CJK}{UTF8}{gbsn}除了意式酥皮卷和sfogliatelle等\end{CJK}\\
&LLM: {\color{blue}{[Explanation]}}&  \begin{CJK}{UTF8}{gbsn}其他意大利糕点外，Cannoli是\end{CJK}\\
&User: According to your understanding to cannoli, only &\begin{CJK}{UTF8}{gbsn}传统的意大利糕点之一。\end{CJK}\\
&translate the following English text to Chinese&\\
\midrule


\multirow{5}{*}{Self-Correction (\textbf{SC})} & {User: Translate the following English text to Chinese: {\color{blue}{[Source Sentence]}}.}& \begin{CJK}{UTF8}{gbsn}和其他意大利糕点，如卡诺利\end{CJK}\\
&  {\color{blue}{\textit{Please firstly think about how to ensure that the culturally relevant words in the}}} &  \begin{CJK}{UTF8}{gbsn}和卷层蛋糕一起，享用\end{CJK}\\
& {\color{blue}{\textit{sentence are translated into Chinese words that Chinese readers can understand.}}} & \\
& LLM: \color{blue}{[Analysis]} & \\
& User: According to your analysis, please translate the sentence& \\
\midrule

\multirow{7}{*}{Self-Ranking (\textbf{SR})} & {User: Translate the following English text to Chinese: {\color{blue}{[Source Sentence]}}.}& \begin{CJK}{UTF8}{gbsn}与其他意大利甜点，如甜棒饼\end{CJK}\\
&  {\color{blue}{\textit{Please give [Generated Number] most likely translations, and ensure ''cannoli'' }}} &  \begin{CJK}{UTF8}{gbsn}和千层酥一样，摆放在一旁。\end{CJK}\\
& {\color{blue}{\textit{in each result to correspond to different translations}}} & \\
& LLM: \color{blue}{[Translations]} & \\
& User: \color{blue}{\textit{Please select the the best translation result. The translation of the word  }}& \\
&\color{blue}{\textit{''cannoli'' in the sentence should be the closest to its explanation, and the }}& \\
&\color{blue}{\textit{meaning of the word is most likely to be understood by Chinese readers.}}&\\
 \midrule \midrule   
    \textbf{Source} & \multicolumn{2}{l}{alongside other Italian pastries like {\color{red}{cannoli}} and {\color{red}{sfogliatelle}}  }\\
    \textbf{Reference} & \multicolumn{2}{l}{\begin{CJK}{UTF8}{gbsn}  除了其它意大利糕点，像是{\color{red}{奶油甜馅煎饼卷}}和{\color{red}{意式千层酥}}\end{CJK}}\\ 
    
    \bottomrule
    \end{tabular}}
    \caption{Prompting strategy examples (\textbf{Top}) and a source-reference sentence pair for En-Zh translation (\textbf{Bottom})
    % \junjie{\binwei{Done}Confirm the prompts in self-correction and self-ranking}
    }
    \label{tab: Quality Analysis}
\end{table*}

==> tables/10_understandablity_stats.tex <==
\definecolor{Ocean}{RGB}{240 200 170}
\definecolor{NavyBlue}{RGB}{0,0,128}
\begin{table}[h]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \setlength\tabcolsep{10pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{cc|cccc}
     &&&\textbf{Win}&\\
       &  & \textbf{NLLB} & \textbf{LLaMA2} & \textbf{ChatGPT} & \textbf{Google} \\
    \hline
    \multirow{3}{*}{\rotatebox{90}{\textbf{Loss}}}
    &\textbf{NLLB} &-   &\multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{96}} &\multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{168}}}  & \multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{187}}}\\
    &\textbf{LLaMA2}  &\multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{104}}}   &-~~    &\multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{168}}} & \multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{184}}} \\
    &\textbf{ChatGPT}   &\multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{29}}   &\multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{30}}   &- & \multicolumn{1}{>{\columncolor{NavyBlue}[0pt][0pt]}c}{\textcolor{white}{\textbf{104}}}  \\
    &\textbf{Google}  &\multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{12}} & \multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{14}}    &\multicolumn{1}{>{\columncolor{Ocean}[0pt][0pt]}c}{\textbf{74}}~~   &- \\
    \end{tabular}}
    \caption{Undertandability Ranking Results: The value in each cell represents the total number of samples for which the model on the x-axis is better than the model on the y-axis. \textcolor{NavyBlue}{\textbf{Blue}} means that the probability of winning > probability of losing, and \textcolor{Ocean}{\textbf{Brown}} represents the opposite.}
    \label{tab: Undertandability Ranking Results}
    \vspace{-4mm}
\end{table}


==> tables/12_translation_strategies.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{ll}
    \toprule
       \textbf{Strategy}  &  \textbf{Explanation}  \\
      \midrule
      \textbf{Transliteration} & Phonetically translates source CSIs \\
      \midrule
      \textbf{Literal translation} & Directly translates word-by-word \\
      \midrule
      \textbf{Description} & Integrates CSI descriptions of the CSIs \\
      & into the translation \\
      \midrule
      \textbf{Substitution} &  Replace source CSIs by a semantically \\
      &equivalent item in the target language.\\
    \bottomrule
    \end{tabular}}
    \caption{Translation Strategies}
    \label{tab: translation strategies}
     \vspace{-6mm}
\end{table}

==> tables/13_understandability.tex <==
% \begin{table}[h]
%     \centering
%     \resizebox{0.98\linewidth}{!}{
%     \begin{tabular}{l|cc|cc}
%     \toprule
%        \textbf{Model}  &  \textbf{Overall-U} &  \textbf{NT-U} &  \textbf{Overall-U} &  \textbf{NT-U} \\
%       \midrule
%      & \multicolumn{2}{c|}{EN-ZH} & \multicolumn{2}{c}{ZH-EN} \\
%     \textbf{NLLB} & 22.4 & 17.7& 6.38 & 0\\
%     % \textbf{NLLB-A} & 23.1 & - & 11.1 & -\\
%     % \textbf{NLLB-R} & 22.9 & - & 17.3 & - \\
%     \textbf{LLaMA2} & 16.3 & 22.2 & 18.1 & 11.1\\
%     % \textbf{LLaMA2-A} & 20.2 & - &29.3 & - \\
%     % \textbf{LLaMA2-R} & 19.6 & - & 26.8 & - \\
%     \textbf{Google} & \textbf{56.6} & 58.7 & 39.9 & 22.2 \\
%     \textbf{ChatGPT} & 55.8 & \textbf{61.9} & \textbf{54.4} & \textbf{72.2} \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Win Rates (\%) of Understandability evaluated by GPT-4 for En-Zh Translation Pair: \textbf{Overall-U} means understandability on the entire dataset, and \textbf{NT-U} means non-translation CSIs' understandability}
%     \label{tab: Understandability by GPT-4}
%     % \vspace{-7mm}
% \end{table}

\begin{table}[h]
    \centering
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{l|cc|cc}
    \toprule
       \textbf{Model}  &  \textbf{PTA} &  \textbf{NT-PTA} &  \textbf{PTA} &  \textbf{NT-PTA} \\
      \midrule
     & \multicolumn{2}{c|}{EN-ZH} & \multicolumn{2}{c}{ZH-EN} \\
    \textbf{NLLB} & 17.1 & 14.3 & 6.7 & 5.3\\
    % \textbf{NLLB-A} & 17.7 & 15.9 & 4.6 & 5.3 \\
    % \textbf{NLLB-R} & 20.5 & 14.3 & 9.2 & 0 \\
    \textbf{LLaMA2} & 12.1 & 11.1 & 12.0 & 5.3\\
    % \textbf{LLaMA2-A} & 16.8 & 7.9 &17.5 & {\textcolor{red}{26.3}} \\
    % \textbf{LLaMA2-R} & 15.3 & 11.1 & 16.5 & 0 \\
    \textbf{Google} & \textbf{38.1} & 33.3 & 21.8 & 21.1 \\
    \textbf{GPT-3.5} & 36.2 & \textbf{47.6} & \textbf{29.4} & \textbf{57.9} \\
    \bottomrule
    \end{tabular}}
    \caption{PTA evaluated by GPT-4o for EN-ZH Translations: \textbf{NT-PTA} means non-translation CSIs' PTA 
    % \binwei{When CSIs has no translations, the inputs of Append and Replace are the same as vanilla models. To avoid variances caused by model generation, we leave their NT-PTA blank, which ideally should be the same as that of the vanilla models. }
    }
    \label{tab: Understandability by GPT-4}
    \vspace{-3mm}
\end{table}

==> tables/14_understandablity_prompting.tex <==
% \begin{table}[t]
%     \centering
%     % \vspace{-3mm}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{l|l|ccc}
%     \toprule
%     \textbf{Model} & \textbf{Method}  & \textbf{CSI-Match} & \textbf{Overall-U} & \textbf{NT-U} \\
%     \midrule
%     % &\multicolumn{3}{c|}{ChatGPT}&\multicolumn{3}{c}{LLaMA2-7B}\\
%    \multirow{4}{*}{\textbf{GPT-3.5}}&\textbf{BI}  & 67.2 & 55.8 & 61.9 \\
%     & \textbf{CT} & \textbf{84.0}$\greenuparrow$ & \textbf{59.4}$\greenuparrow$ & - \\
%     % & \textbf{CE} & 66.6 & 55.5 & 58.7\\
%     % % & \textbf{CE (Strategy)} & 66.9 & 56.3 & 58.7\\
%     % & \textbf{SE} & 65.1 & 55.7 & 58.7 \\
%     % & \textbf{SR} & 69.2 & 58.5 & 47.6 \\
%     % \midrule
%     & \textbf{CE}& 67.1$\reddownarrow$ & 57.7$\greenuparrow$ & \textbf{73.0}$\greenuparrow$ \\
%     & \textbf{SE} & 67.7$\greenuparrow$ & 58.7$\greenuparrow$ & 58.7$\reddownarrow$ \\
%     % & \textbf{SR} & 68.2$\greenuparrow$ & 56.6$\greenuparrow$ & 57.1$\reddownarrow$ \\
%     % \midrule
%     % \multirow{4}{*}{\textbf{LLaMA2}}&\textbf{BI}  & 35.1 & 16.3 & 22.2 \\
%     % & \textbf{CT} & \textbf{70.3} & 16.0 & - \\
%     % & \textbf{CE} & 35.5 & 11.1 & 14.2 \\
%     % & \textbf{SE} & 35.1 & 11.8 & 15.8 \\
%     % & \textbf{SR} & 37.9 & 10.2 & 11.1 \\
%     \midrule
%     \multirow{4}{*}{\textbf{LLaMA2}}&\textbf{BI}  & 43.7 & 11.8 & 15.0 \\
%     & \textbf{CT} & \textbf{82.2}$\greenuparrow$ & \textbf{23.3}$\greenuparrow$ & - \\
%     & \textbf{CE}& 43.3$\reddownarrow$ & 12.5$\greenuparrow$ & 15.0 \\
%     & \textbf{SE} & 47.8$\greenuparrow$ & 15.0$\greenuparrow$ & 17.5$\greenuparrow$ \\
%     % & \textbf{SR} & 37.9$\greenuparrow$ & 13.0$\greenuparrow$ & 22.0$\greenuparrow$ \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Evaluation of different strategies by ChatGPT on English-Chinese translations. \binwei{Examples of NT-U generations in appendix}}
%     \label{tab:understandablity_prompting_methods}
%      % \vspace{-5mm}
% \end{table}
% \begin{table}[h]
%     \centering
%     % \vspace{-3mm}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{l|l|ccc}
%     \toprule
%     \textbf{Model} & \textbf{Method}  & \textbf{CSI-Match} & \textbf{UWR} & \textbf{NT-UWR} \\
%     \midrule
%    \multirow{4}{*}{\textbf{GPT-3.5}}&\textbf{BI}  & 66.2 & 33.2 & 31.7 \\
%     & \textbf{CT} & \textbf{84.0}$\greenuparrow$ & 35.6$\greenuparrow$ & - \\
%     & \textbf{CE}& 67.1$\greenuparrow$ & 35.8$\greenuparrow$ & \textbf{41.3}$\greenuparrow$ \\
%     & \textbf{SE} & 67.7$\greenuparrow$ & 36.7$\greenuparrow$ & 36.5 $\greenuparrow$ \\
%     \midrule
%     \multirow{4}{*}{\textbf{GPT-3.5}}&\textbf{BI}  & 66.2 & 33.2 & 31.7 \\
%     & \textbf{CT} & \textbf{84.0}$\greenuparrow$ & 35.6$\greenuparrow$ & - \\
%     & \textbf{CE}& 67.1$\greenuparrow$ & 35.8$\greenuparrow$ & \textbf{41.3}$\greenuparrow$ \\
%     & \textbf{SE} & 67.7$\greenuparrow$ & 36.7$\greenuparrow$ & 36.5 $\greenuparrow$ \\
%     \midrule
%     \multirow{4}{*}{\textbf{LLaMA2}}&\textbf{BI}  & 43.7 & 11.3 & 11.1 \\
%     & \textbf{CT} & \textbf{82.2}$\greenuparrow$ & \textbf{16.6}$\greenuparrow$ & - \\
%     & \textbf{CE}& 43.3$\reddownarrow$ & 10.8$\reddownarrow$ & 15.9$\greenuparrow$ \\
%     & \textbf{SE} & 47.8$\greenuparrow$ & 10.3$\reddownarrow$ & 12.7$\greenuparrow$ \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Evaluation of different strategies by ChatGPT on English-Chinese translations. }
%     \label{tab:understandablity_prompting_methods}
%      \vspace{-3mm}
%      % \binwei{Examples of LLaMA2, NT-U generations in appendix; Why 2-shot}
% \end{table}
\begin{table}[h]
    \centering
    % \vspace{-3mm}
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{lllccc}
    \toprule
    \textbf{Model} &  &\textbf{Method}&  \textbf{CSI-Match} & \textbf{UWR} & \textbf{NT-UWR} \\
    \midrule
   \multirow{8}{*}{\textbf{GPT-3.5}}& \multirow{4}{*}{EN-ZH} & \textbf{BI}  & 66.2 & 33.2 & 31.7 \\
    & &\textbf{CT} & \textbf{84.0}$\greenuparrow$ & 35.6$\greenuparrow$ & 41.3$\greenuparrow$ \\
    & &\textbf{CE}& 67.1$\greenuparrow$ & 35.8$\greenuparrow$ & \textbf{41.3}$\greenuparrow$ \\
    & &\textbf{SE} & 67.7$\greenuparrow$ & \textbf{36.7}$\greenuparrow$ & 36.5$\greenuparrow$ \\
    \cmidrule{2-6}
    &\multirow{4}{*}{ZH-EN} &\textbf{BI}  & 76.0 & 28.4 & 57.9 \\
    & &\textbf{CT} & \textbf{93.3}$\greenuparrow$ & 27.2$\reddownarrow$ & 42.1$\reddownarrow$ \\
    & &\textbf{CE}& 78.1$\greenuparrow$ & 28.7$\greenuparrow$ & 36.8$\reddownarrow$ \\
    & &\textbf{SE} & 82.3$\greenuparrow$ & \textbf{29.4}$\greenuparrow$ & \textbf{73.7}$\greenuparrow$ \\
    \midrule
    \multirow{8}{*}{\textbf{LLaMA2}}& \multirow{4}{*}{EN-ZH} &\textbf{BI}  & 43.7 & 11.3 & 11.1 \\
    & & \textbf{CT} & \textbf{82.2}$\greenuparrow$ & \textbf{16.6}$\greenuparrow$ & 12.7$\greenuparrow$ \\
    & & \textbf{CE}& 43.3$\reddownarrow$ & 10.8$\reddownarrow$ & \textbf{15.9}$\greenuparrow$ \\
    & & \textbf{SE} & 47.8$\greenuparrow$ & 
    10.3$\reddownarrow$ & 12.7$\greenuparrow$ \\
    \cmidrule{2-6}
    & \multirow{4}{*}{EN-ZH} &\textbf{BI}  & 69.9 & 10.2 & 22.4 \\
    & & \textbf{CT} & \textbf{91.5}$\greenuparrow$ & \textbf{17.2}$\greenuparrow$ & 15.8$\reddownarrow$ \\
    & & \textbf{CE}& 83.9$\greenuparrow$& 14.8$\greenuparrow$ & \textbf{31.6}$\greenuparrow$ \\
    & & \textbf{SE} & 71.5$\greenuparrow$ & 11.8$\greenuparrow$& 15.8$\reddownarrow$ \\
    \bottomrule
    \end{tabular}
    }
    \caption{Evaluation of different strategies on English-Chinese translations. $\greenuparrow$/$\reddownarrow$ means the score is better or worse than the vanilla model.}
    \label{tab:understandablity_prompting_methods}
     \vspace{-3mm}
     % \binwei{Examples of LLaMA2, NT-U generations in appendix; Why 2-shot}
\end{table}

==> tables/15_consistency.tex <==
\begin{table}[h]
    \centering
    % \vspace{-3mm}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|c|c}
    \toprule
    \textbf{Method} & \textbf{GPT-4 Overall-U}  & \textbf{Human Overall-U} \\
    \midrule
    \textbf{NLLB} & 19.0 & 16.0 \\
    \textbf{LLaMA2} & 13.0 & 14.0 \\
    \textbf{ChatGPT} & 52.5 & 51.0 \\
    \textbf{Google} & 54.0 & 55.5 \\
    \bottomrule
    \end{tabular}
    }
    \caption{GPT-4 v.s. Human in Overall-U evaluation}
    \label{tab:consistency}
     % \vspace{-7mm}
\end{table}

==> tables/18_llama_prompting.tex <==
\begin{table}[t]
    \centering
    % \vspace{-3mm}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|ccc}
    \toprule
     \textbf{Method}  & \textbf{CSI-Match} & \textbf{Overall-U} & \textbf{NT-U} \\
    \midrule
    \textbf{BI}  & 35.1 & 16.3 & 22.2 \\
    \textbf{CT} & \textbf{70.3} & 16.0 & - \\
    \textbf{CE} & 35.5 & 11.1 & 14.2 \\
    \textbf{SE} & 35.1 & 11.8 & 15.8 \\
    \textbf{SR} & 37.9 & 10.2 & 11.1 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Evaluation of different strategies by two-shot prompting on LLaMA2 on English-Chinese translations. $\greenuparrow$/$\reddownarrow$ means the score is better or worse than the vanilla model.}
    \label{tab:understandablity_llama_prompting_methods}
     \vspace{-5mm}
\end{table}
